Measuring HTTP/3: Adoption and Performance

The third version of the Hypertext Transfer Protocol (HTTP) is currently in its final standardization phase by the IETF. Besides better security and increased flexibility, it promises benefits in terms of performance. HTTP/3 adopts a more efficient header compression schema and replaces TCP with QUIC, a transport protocol carried over UDP, originally proposed by Google and currently under standardization too. Although HTTP/3 early implementations already exist and some websites announce its support, it has been subject to few studies. In this work, we provide a first measurement study on HTTP/3. We testify how, during 2020, it has been adopted by some of the leading Internet companies such as Google, Facebook and Cloudflare. We run a large-scale measurement campaign toward thousands of websites adopting HTTP/3, aiming at understanding to what extent it achieves better performance than HTTP/2. We find that adopting websites often host most web page objects on third-party servers, which support only HTTP/2 or even HTTP/1.1. Our experiments show that HTTP/3 provides sizable benefits only in scenarios with high latency or very poor bandwidth. Despite the adoption of QUIC, we do not find benefits in case of high packet loss, but we observe large diversity across website providers' infrastructures.

==> makefile <==
DOC=main

all:
	pdflatex $(DOC)
	bibtex   $(DOC)
	pdflatex $(DOC)
	pdflatex $(DOC)

clean:
	find . -name '*~' -exec rm -f {} \;
	find . -name '*.aux' -exec rm -f {} \;
	rm -f texput.log $(DOC).log $(DOC).ps $(DOC).toc $(DOC).lo* $(DOC).bbl $(DOC).blg $(DOC).dvi $(DOC).out $(DOC).synctex.gz diff.bbl diff.blg

zip: ${sources} ${pdffiles}
	rm -f $(DOC).zip && zip -r $(DOC).zip *.tex *.bib *.bbl *.cls figures Makefile makefile

diff:
		latexdiff -c submission_version/latexdiff_conf.txt \
							--preamble=submission_version/latexdiff_preamble_old.tex \
		          --exclude-textcmd="subsection" \
	            --flatten submission_version/main.tex main.tex > diff.tex
		#pdflatex diff
		#bibtex diff
		pdflatex diff
		pdflatex diff

